Hierarchical sparse recovery from hierarchically structured measurements with application to massive random access

A new family of operators, coined hierarchical measurement operators, is introduced and discussed within the well-known hierarchical sparse recovery framework. Such operator is a composition of block and mixing operations and notably contains the Kronecker product as a special case. Results on their hierarchical restricted isometry property (HiRIP) are derived, generalizing prior work on recovery of hierarchically sparse signals from Kronecker-structured linear measurements. Specifically, these results show that, very surprisingly, sparsity properties of the block and mixing part can be traded against each other. The measurement structure is well-motivated by a massive random access channel design in communication engineering. Numerical evaluation of user detection rates demonstrate the huge benefit of the theoretical framework.

==> Nonconstant Kronecker Conference/macros_flinth.tex <==
 %\textwidth  6.8in \textheight 8.5in
%\topmargin0cm \oddsidemargin0cm \evensidemargin0cm



\usepackage{hyperref}
\usepackage{verbatim} %to allow long "comment-out-'s"

\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amssymb}
\usepackage{ textcomp } %Promille sign
\usepackage{color}
\usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage{multicol}
\usepackage{hyperref}
\usepackage{amsopn}

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}

\usepackage{multicol}


%\usepackage{algorithm}
%\usepackage{algorithmic} 
%\usepackage{algpseudocode}


%\usepackage{chngcntr}
%\usepackage{apptools}
%\AtAppendix{\counterwithin{lem}{section}}

\newcommand{\dotrule}[1]{%
   \parbox[t]{#1}{\dotfill}}




\newcommand{\C}{\mathbb{C}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\spann}{\mathrm{span}}


\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calY}{\mathcal{Y}}

\newcommand{\frakA}{\mathfrak{A}}

\newcommand{\scrS}{\mathscr{S}}

\newcommand{\vphi}{\varphi}


\newcommand{\abs}[1]{\left\vert #1 \right\vert}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\newcommand{\abss}[1]{\left\vert #1 \right\vert}
\newcommand{\normm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\set}[1]{\left\lbrace #1\right\rbrace}
\newcommand{\sse}{\subseteq}
\newcommand{\sprod}[1]{\left\langle #1 \right\rangle}

\newcommand{\sph}{\mathbb{S}}
\newcommand{\gl}{\mthfrak{gl}}

%Wahrscheinlichkeitstheorie
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\prob}[1]{\mathbb{P}\left( \text{#1}\right)}
\newcommand{\prb}[1]{\mathbb{P}\left( #1 \right)}
\newcommand{\erw}[1]{\mathbb{E}\left( #1 \right)}
\newcommand{\uniform}[1]{\mathcal{U}\left( #1 \right)}
\newcommand{\impl}{\Rightarrow}
\newcommand{\alg}{\mathfrak{A}}

\usepackage{dsfont}
%\newcommand{\ind}{\mathds{1}}
%\newcommand{\1}{\text{1}}
%\newcommand{\muExp}[1]{{#1}^{\wedge \mu}}
%\newcommand{\matleq}{\preccurlyeq}
%\newcommand{\matgeq}{\succcurlyeq}
%\newcommand{\matleqdef}{\prec}
%\newcommand{\matgeqdef}{\succ}

\newcommand{\geqsim}{\gtrsim}
\newcommand{\leqsim}{\lesssim}

%\newcommand{\wto}{\rightharpoonup}
%\newcommand{\wstarto}{\stackrel{*}{\wto}}

%\newcommand{\hatH}{\widehat{H}}
%\newcommand{\hatZ}{\widehat{Z}}
%\newcommand{\hatsigma}{\widehat{\sigma}}
%\newcommand{\hatphi}{\widehat{\phi}}

%conv,cone,argmin uzw.
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\clonv}{\overline{conv}}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\qri}{qri}
\DeclareMathOperator{\vertx}{vert}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rd}{rd}
\DeclareMathOperator{\distinf}{dist_{\infty}}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Id}{Id}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\DeclareMathOperator{\ran}{ran}
\DeclareMathOperator{\pos}{pos}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\mat}{mat}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sym}{sym}
\DeclareMathOperator{\dom}{dom}
\newcommand{\hess}{\mathrm{hess}}

\DeclareMathOperator{\ri}{ri}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}


\newcommand{\st}{\text{ subject to }}


\newtheorem{lem}{Lemma}
\newtheorem{prop}[lem]{Proposition}

\newtheorem{theo}[lem]{Theorem}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{assumption}{Assumption}

\newtheorem{defi}{Definition}
\newtheorem{rem}{Remark}


\theoremstyle{definition}
%\newtheorem{example}[lem]{Example}

\numberwithin{lem}{section}

\usepackage{etoolbox}
\let\bbordermatrix\bordermatrix
\patchcmd{\bbordermatrix}{8.75}{4.75}{}{}
\patchcmd{\bbordermatrix}{\left(}{\left[}{}{}
\patchcmd{\bbordermatrix}{\right)}{\right]}{}{}

\newcommand{\todo}[1]{{\color{red}  \bf TODO: #1}}

